Reliable approximation of separatrix manifolds in competition models with safety niches

In dynamical systems saddle points partition the domain into basins of attractions of the remaining locally stable equilibria. This situation is rather common especially in population dynamics models, like prey-predator or competition systems. Focusing on squirrels population models with niche, in this paper we design algorithms for the detection and the refinement of points lying on the separatrix manifold partitioning the phase space. We consider both the two populations and the three populations cases. To reconstruct the separatrix curve and surface, we apply the Partition of Unity method, which makes use of Wendland's functions as local approximants.

==> psfrag.sty.tex <==
%%
%% This is file `psfrag.sty',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% psfrag.dtx  (with options: `package')
%% 
%% Copyright (c) 1996 Craig Barratt, Michael C. Grant, and David Carlisle.
%% All rights reserved.
%% 
%% This file is part of the PSfrag package.
%% 
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesPackage{psfrag}[1998/04/11 v3.04 PSfrag (MCG)]
\newif\ifpfg@compat
\newif\ifpfg@prepass
\newif\ifpfg@debug \pfg@debugfalse
\if@compatibility
  \pfg@compattrue\pfg@prepasstrue
\else
  \pfg@compatfalse\pfg@prepassfalse
\fi
\def\psfragscanon{\pfg@prepasstrue}
\def\psfragscanoff{\pfg@prepassfalse}
\def\psfragdebugon{\pfg@debugtrue}
\def\psfragdebugoff{\pfg@debugfalse}
\DeclareOption{scanall}{\pfg@prepasstrue}
\DeclareOption{2emode}{\pfg@compatfalse\pfg@prepassfalse}
\DeclareOption{209mode}{\pfg@compattrue\pfg@prepasstrue}
\DeclareOption{debugshow}{\pfg@debugtrue
                         \PassOptionsToPackage\CurrentOption{graphics}}
\DeclareOption*{\PassOptionsToPackage\CurrentOption{graphics}}
\ProcessOptions
\RequirePackage{graphics}
\providecommand\Gin@PS@file@header[1]{\AtBeginDvi{\special{header=#1}}}
\Gin@PS@file@header{psfrag.pro}
\def\pfg@orient{1}
\def\@tempa{dvipsone.def}\ifx\Gin@driver\@tempa\def\pfg@orient{-1}\fi%
\def\@tempa{dvips.def}\ifx\Gin@driver\@tempa\def\pfg@orient{-1}\fi%
\def\@tempa{textures.def}\ifx\Gin@driver\@tempa\def\pfg@orient{-1}\fi%
\let\pfg@epsfbox\epsfbox
\let\pfg@Ginclude@eps\Ginclude@eps
\newcount\pfg@pcount \pfg@pcount=\z@
\newcount\pfg@scount \pfg@scount=\z@
\def\epsfbox#1{%
    \begingroup
    \let\Ginclude@eps\pfg@Ginclude@eps
    \let\epsfbox\pfg@epsfbox
    \ifpfg@prepass\pfg@scan{#1}\fi
    \ifnum\pfg@scount>\z@\pfg@hidestart\fi
    \pfg@epsfbox{#1}%
    \ifnum\pfg@scount>\z@\pfg@hideend\fi
    \endgroup}
\def\Ginclude@eps#1{%
    \begingroup
    \let\Ginclude@eps\pfg@Ginclude@eps
    \let\epsfbox\pfg@epsfbox
    \ifpfg@prepass\pfg@scan{#1}\fi
    \ifnum\pfg@scount>\z@\pfg@hidestart\fi
    \pfg@Ginclude@eps{#1}%
    \ifnum\pfg@scount>\z@\pfg@hideend\fi
    \endgroup}
\newenvironment{psfrags}{\ignorespaces}{\global\@ignoretrue}
\ifpfg@compat
\def\psfragspecial#1#2#3#4#5#6{%
   \PackageError{PSfrag}%
     {\string\psfragspecial no longer implemented.}{}}
\fi
\newif\ifpfg@star
\def\psfrag{\@ifstar{\pfg@startrue\@psfraga}{\pfg@starfalse\@psfraga}}
\def\@psfraga{\begingroup
   \@makeother\"\@makeother\*\@makeother\!\@makeother\~%
   \@makeother\:\@makeother\\\@makeother\%\@makeother\#%
   \@makeother\ \@psfragb}
\ifpfg@compat
\def\@psfragb#1{\xdef\@gtempa{#1}\endgroup
                \@ifnextchar[{\@psfragc{\@gtempa}}%
                             {\@psfrag{\@gtempa}[bl][bl][1][0]}}
\def\@psfragc#1[#2]{\@ifnextchar [{\@psfragd{#1}[#2]}%
                                  {\@psfrag{#1}[#2][bl][1][0]}}
\else
\def\@psfragb#1{\xdef\@gtempa{#1}\endgroup
                \@ifnextchar [{\@psfragc{\@gtempa}}%
                              {\@psfrag{\@gtempa}[Bl][Bl][1][0]}}
\def\@psfragc#1[#2]{\@ifnextchar [{\@psfragd{#1}[#2]}%
                                  {\@psfrag{#1}[#2][Bl][1][0]}}
\fi
\def\@psfragd#1[#2][#3]{\@ifnextchar [{\@psfrage{#1}[#2][#3]}%
                                      {\@psfrag{#1}[#2][#3][1][0]}}
\def\@psfrage#1[#2][#3][#4]{\@ifnextchar [{\@psfrag{#1}[#2][#3][#4]}%
                                       {\@psfrag{#1}[#2][#3][#4][0]}}
\def\pfg@newstring#1.#2{%
    \@nameedef{pfg@using@#2}{#1}%
    \pfg@starfalse\advance\pfg@scount\@ne}
\def\@psfrag#1{%
    \@ifundefined{pfg@using@#1}%
      {\expandafter\pfg@newstring\the\pfg@scount.{#1}}%
      {}%
    \edef\@tempa{\@nameuse{pfg@using@#1}}%
    \expandafter\@@psfrag\@tempa.{#1}}
\def\@@psfrag{\expandafter\@@@psfrag\the\pfg@pcount.}
\def\@nameedef#1#2{\expandafter\edef\csname #1\endcsname{#2}}
\def\@@@psfrag#1.#2.#3[#4][#5][#6][#7]#8{%
    \advance\pfg@pcount\@ne
    \ifpfg@star\else\@nameedef{pfg@align@#2}{(#3)[}\fi
    \@nameedef{pfg@align@#2}{\@nameuse{pfg@align@#2}[#1(#5)#6 #7]}%
    \@namedef{pfg@place@#1}{\pfg@@place{#1}{#4}{#8}}\ignorespaces}
\def\pfg@align#1.{\@nameuse{pfg@align@#1}}
\def\pfg@place#1.{\@nameuse{pfg@place@#1}}
\def\pfg@hidestart{%
    \def\pfg@{}\count@=\z@\loop\ifnum\count@<\pfg@scount
        \toks@=\expandafter{\expandafter\pfg@align\the\count@.}%
        \edef\pfg@{\pfg@\the\toks@]}%
        \advance\count@ by\@ne\repeat
    \Gin@PS@raw{/PSfrag where{pop\pfg@\the\pfg@scount\space
                \ifpfg@debug1\else0\fi\space\pfg@orient/Begin
                PSfrag}{userdict /PSfrag{pop}put}ifelse}}
\def\pfg@hideend{%
    \Gin@PS@raw{/End PSfrag}%
    \vbox to\z@{\vss
        \Gin@PS@raw{/Hide PSfrag}%
        \hbox to\z@{\hss \raisebox{\depth}{%
            \underline{PSfrag replacements}}}%
        \Gin@PS@raw{/Unhide PSfrag}%
        \count@=\z@\loop\ifnum\count@<\pfg@pcount
            \expandafter\pfg@place\the\count@.%
            \advance\count@ by\@ne\repeat}}
\let\pfg@dp\leftmargini\let\pfg@wd\leftmarginii
\let\pfg@dx\leftmarginiii\let\pfg@dy\leftmarginiv
\edef\pfg@bchar{ \string{ }
\edef\pfg@echar{ \string} }
\def\pfg@@place#1#2#3{\begingroup
    \sbox\z@{#3}%
    \dimen@=\ht\z@ \advance\dimen@ by\dp\z@%
    \pfg@wd=0.5\wd\z@\pfg@dp=0.5\dimen@
    \pfg@dx=\pfg@wd\pfg@dy=\pfg@dp
    \@tfor\@tempa:=#2\do{%
        \if l\@tempa \pfg@dx=\z@    \pfg@wd=\wd\z@ \else
        \if r\@tempa \pfg@dx=\wd\z@ \pfg@wd=\z@    \else
        \if b\@tempa \pfg@dy=\z@    \pfg@dp=\z@    \else
        \if t\@tempa \pfg@dy=\dimen@\pfg@dp=\dimen@\else
        \if B\@tempa \pfg@dy=\dp\z@ \pfg@dp=\dp\z@ \fi\fi\fi\fi\fi}%
    \setbox\z@\hbox to\z@{\hskip-\pfg@dx\box\z@\hss}%
    \setbox\z@\vbox to\z@{\vss\box\z@\vskip-\pfg@dy}%
    \vbox to\dimen@{\vss\hbox to\z@{\hss
        \Gin@PS@raw{\pfg@bchar}\box\z@
        \Gin@PS@raw{\pfg@echar#1/Place PSfrag}%
        \hskip\pfg@wd}\vskip\pfg@dp}%
    \endgroup}
\newwrite\pfg@temp
\def\pfg@scan#1{\begingroup
    \@tempcnta\z@
    \loop
    \ifnum\@tempcnta<\@xxxii
        \catcode\@tempcnta12 \advance\@tempcnta\@ne
    \repeat
    \let\do\@makeother\dospecials\catcode`\ 10 %
    \catcode`\{=1\catcode`\}=2\catcode127=12 %
    \catcode`\\=\active\catcode\endlinechar5 %
    \immediate\openout\pfg@temp=\jobname.pfg %
    \immediate\openin\@inputcheck=#1 %
    \ifeof\@inputcheck
      \PackageWarning{psfrag}{Could not scan #1...}\endgroup
    \else
      \message{<psfrag:#1>}%
      \@tempswatrue
      \loop
        \ifeof\@inputcheck
          \@tempswafalse
        \else
          \read\@inputcheck to\@tempa
          \expandafter\pfg@find\@tempa{\@nil}%
        \fi
      \if@tempswa
      \repeat
      \closein\@inputcheck
    \fi
    \immediate\closeout\pfg@temp
    \endgroup
    \@input{\jobname.pfg}}
\long\def\pfg@find#1#{\pfg@finda{#1}}
\begingroup
  \lccode`\~=`\\
  \lowercase{\endgroup
\long\def\pfg@finda#1#2{%
  \def\@tempa{#2}%
  \ifx\@tempa\@nnil
  \else
    \pfg@findb#1(~~tex(~~tex%
  \fi}
\long\def\pfg@findb#1(~~tex#2(~~tex#3\fi{%
  \fi
  \ifx\box#3\box
  \else
     {\let~\string
        \edef\@tempb{\@tempa}%
      \let~\relax
        \immediate\write\pfg@temp{%
          \string\psfrag\space
            {\string\\tex#2{\@tempa}}#2\@percentchar
          ^^J\@spaces\@spaces{\@tempb}\@percentchar}}%
    \let\@tempa\@empty
  \fi
  \expandafter\pfg@find\@tempa}
}
\endinput
%%
%% End of file `psfrag.sty'.

